FLEXI: A high order discontinuous Galerkin framework for hyperbolic-parabolic conservation laws

High order (HO) schemes are attractive candidates for the numerical solution of multiscale problems occurring in fluid dynamics and related disciplines. Among the HO discretization variants, discontinuous Galerkin schemes offer a collection of advantageous features which have lead to a strong increase in interest in them and related formulations in the last decade. The methods have matured sufficiently to be of practical use for a range of problems, for example in direct numerical and large eddy simulation of turbulence. However, in order to take full advantage of the potential benefits of these methods, all steps in the simulation chain must be designed and executed with HO in mind. Especially in this area, many commercially available closed-source solutions fall short. In this work, we therefor present the FLEXI framework, a HO consistent, open-source simulation tool chain for solving the compressible Navier-Stokes equations in a high performance computing setting. We describe the numerical algorithms and implementation details and give an overview of the features and capabilities of all parts of the framework. Beyond these technical details, we also discuss the important, but often overlooked issues of code stability, reproducibility and user-friendliness. The benefits gained by developing an open-source framework are discussed, with a particular focus on usability for the open-source community. We close with sample applications that demonstrate the wide range of use cases and the expandability of FLEXI and an overview of current and future developments.

==> coordimg.tex <==
\usepackage{tikz}
\usepackage{xkeyval}
\usepackage{pgfplots}
\usetikzlibrary{calc}
\usetikzlibrary{fpu}

\makeatletter
\newcommand{\coordimg}{\begingroup
  \catcode`_=12 \coordimgA}
% Bilder mit Koordinatenachsen versehen:
% Usage:
%   mit '\def\scale{5}' vor dem tikzpicture global die Skalierung festlegen,
%   oder halt den Parameter scale benutzen
%   
%   \coordimg[OPTIONEN]{LEGENDE.png} um Image zu plotten: 
%
%   Parameter:
%     scale:     Skalierung
%     x/ypos:    x,y Position im tikzpicture
%     xmin/xmax: minimaler und maximaler Koordinaten in x-Richtung 
%     ymin/ymax: minimaler und maximaler Koordinaten in y-Richtung 
%     x/ytics:   Schrittweite der Beschriftung in x/y-Richtung
%     x/ymtics:  Mikroschrittweite in x/y-Richtung 
%     x/yside:   Position der tics (left/right oder top/bottom)
\define@key{coordimg}{scale}{\def\ci@scale{#1}}
\define@key{coordimg}{xpos}{\def\ci@xpos{#1}}
\define@key{coordimg}{ypos}{\def\ci@ypos{#1}}
\define@key{coordimg}{xmax}{\def\ci@xmax{#1}}
\define@key{coordimg}{ymax}{\def\ci@ymax{#1}}
\define@key{coordimg}{xmin}{\def\ci@xmin{#1}}
\define@key{coordimg}{ymin}{\def\ci@ymin{#1}}
\define@key{coordimg}{xtics}{\def\ci@xtics{#1}}
\define@key{coordimg}{ytics}{\def\ci@ytics{#1}}
\define@key{coordimg}{xmtics}{\def\ci@xmtics{#1}}
\define@key{coordimg}{ymtics}{\def\ci@ymtics{#1}}
\define@choicekey{coordimg}{xside}[\val\xnr]{bottom,top,none}{
   \ifcase\xnr\relax
      \def\ci@yplus{0}
      \def\ci@yanchor{north}
      \def\ci@yfac{-1}
   \or
      \def\ci@yplus{\height}
      \def\ci@yanchor{south}
      \def\ci@yfac{1}
   \or 
      \def\ci@yplus{-1}
   \fi
}{ }
\define@choicekey{coordimg}{yside}[\val\ynr]{left,right,none}{
   \ifcase\ynr\relax
      \def\ci@xplus{0}
      \def\ci@xanchor{east}
      \def\ci@xfac{-1}
   \or
      \def\ci@xplus{\width}
      \def\ci@xanchor{west}
      \def\ci@xfac{1}
   \or
      \def\ci@xplus{-1}
   \fi
}{ }

\newcommand{\coordimgA}[2][]{
   \setkeys{coordimg}{scale=4,xpos=0,ypos=0,xtics=1,ytics=1,xside=bottom,yside=left} % set default key values
   \@ifundefined{scale}{}{\setkeys{coordimg}{scale=\scale}}
   \setkeys{coordimg}{#1} % set new keys

   \pgfmathsetmacro{\width}{(\ci@xmax-\ci@xmin)}
   \pgfmathsetmacro{\height}{(\ci@ymax-\ci@ymin)}
   \pgfmathsetmacro{\imagewidth}{\ci@scale * \width}
   \pgfmathsetmacro{\imageheight}{\ci@scale * \height}
   \node[anchor=south west,inner sep=0] (img) at (\ci@xpos,\ci@ypos) {\includegraphics[width=\imagewidth cm,height=\imageheight cm]{#2}};
      

   % x-axis
   \ifthenelse{\equal{\ci@yplus}{-1}} {
   }{
      % draw line
      \draw ($(\ci@xpos, \ci@ypos+\ci@yplus)$) -- coordinate (x axis mid) ++(\width,0);
      %major ticks
      \pgfmathsetmacro{\xtics}{(\ci@xmin+\ci@xtics)}
      \foreach \x in {\ci@xmin,\xtics,...,\ci@xmax} { 
         \draw ($(\ci@xpos+\x-\ci@xmin,\ci@ypos+\ci@yplus)$) -- ++(0,5pt*\ci@yfac) node[anchor=\ci@yanchor] {
            \pgfmathparse{\x}\pgfmathprintnumber{\pgfmathresult}};
      }
      % minor ticks
      \@ifundefined{ci@xmtics}{}{
         \pgfmathsetmacro{\xmtics}{(\ci@xmin+\ci@xmtics)}
         \pgfmathsetmacro{\mpt}{ceil((\ci@xtics-0.01*\ci@xmtics)/\ci@xmtics)} % miniticks per ticks -1
         \pgfmathsetmacro{\ntics}{ceil(\width/(\ci@xmtics))}                 % number of miniticks 
         \foreach \x [count=\i] in {\ci@xmin,\xmtics,...,\ci@xmax}  { 
            \pgfmathparse{mod(\i-1,\mpt) > 0 ? 1 : 0}
            \ifthenelse{\equal{\pgfmathresult}{1}}{
               \draw ($(\ci@xpos+\x-\ci@xmin,\ci@ypos+\ci@yplus)$) -- ++(0,2pt*\ci@yfac);
            }{
            }
         }
      }
   }

   % y-axis
   \ifthenelse{\equal{\ci@xplus}{-1}} {
   }{
      % draw line
      \draw ($(\ci@xpos+\ci@xplus, \ci@ypos)$) -- coordinate (y axis mid) ++(0,\height);
      %major ticks
      \pgfmathsetmacro{\ytics}{(\ci@ymin+\ci@ytics)}
      \foreach \y in {\ci@ymin,\ytics,...,\ci@ymax} { 
         \draw ($(\ci@xpos+\ci@xplus,\ci@ypos+\y-\ci@ymin)$) -- ++(5pt*\ci@xfac,0) node[anchor=\ci@xanchor] {
            \pgfmathparse{\y}\pgfmathprintnumber{\pgfmathresult}};
      }
      % minor ticks
      \@ifundefined{ci@ymtics}{}{
         \pgfmathsetmacro{\ymtics}{(\ci@ymin+\ci@ymtics)}
         \pgfmathsetmacro{\mpt}{ceil((\ci@ytics-0.01*\ci@ymtics)/\ci@ymtics)} % miniticks per ticks -1
         \pgfmathsetmacro{\ntics}{ceil(\height/(\ci@ymtics))}                 % number of miniticks 
         \foreach \y [count=\i] in {\ci@ymin,\ymtics,...,\ci@ymax}{ 
            \pgfmathparse{mod(\i-1,\mpt) > 0 ? 1 : 0}
            \ifthenelse{\equal{\pgfmathresult}{1}}{
               \draw ($(\ci@xpos+\ci@xplus,\ci@ypos+\y-\ci@ymin)$) -- ++(2pt*\ci@xfac,0);
            }{
            }
         }
      }
   }

\endgroup
}
\makeatother

\makeatletter
\newcommand{\coordlegend}{\begingroup
  \catcode`_=12 \coordlegendA}
% Legende
% Usage:
%   mit '\def\scale{5}' vor dem tikzpicture global die Skalierung festlegen,
%   oder halt den Parameter scale benutzen
%   
%   \coordlegend[OPTIONEN]{LEGENDE.png} um Legende zu plotten: 
%
%   Parameter:
%     scale:   Skalierung
%     x/ypos:  x,y Position im tikzpicture
%     min/max: minimaler und maximaler Werte der Legende
%     width:   Breite der Legende => horizontale Legende  (width darf nicht angegeben werden)
%     height:  Hoehe der Legende  => vertikale Legende    (height darf nicht angegeben werden)
%     tics:    Schrittweite der Beschriftung
%     mtics:   Mikroschrittweite
%     label:   Label (Name der Variable)
\define@key{coordlegend}{scale}{\def\ci@scale{#1}}
\define@key{coordlegend}{xpos}{\def\ci@xpos{#1}}
\define@key{coordlegend}{ypos}{\def\ci@ypos{#1}}
\define@key{coordlegend}{min}{\def\ci@min{#1}}
\define@key{coordlegend}{max}{\def\ci@max{#1}}
\define@key{coordlegend}{height}{\def\ci@height{#1}}
\define@key{coordlegend}{width}{\def\ci@width{#1}}
\define@key{coordlegend}{tics}{\def\ci@tics{#1}}
\define@key{coordlegend}{mtics}{\def\ci@mtics{#1}}
\define@key{coordlegend}{label}{\def\ci@label{#1}}
%\define@key
\newcommand{\coordlegendA}[2][]{
   \setkeys{coordlegend}{scale=4,xpos=0,ypos=0,tics=1} % set default key values
   \@ifundefined{scale}{}{\setkeys{coordlegend}{scale=\scale}}
   \setkeys{coordlegend}{#1} % set new keys

   \@ifundefined{ci@height}{
      % horizontal
      \pgfmathsetmacro{\ci@height}{0};
      \pgfmathsetmacro{\imagesize}{\ci@scale * \ci@width};
      \def\ci@imageanchor{south west};
      \def\ci@imagesizename{width};
      \def\ci@ticksanchor{north};
      \def\ci@mtdx{0};     % major tick delta x
      \def\ci@mtdy{2.5pt}; % major tick delta y
      \def\ci@tdx{0};      % minor tick delta x
      \def\ci@tdy{1pt};    % minor tick delta y
      \def\ci@facx{1};
      \def\ci@facy{0};
      \def\ci@legendanchor{east};
   }{
      % vertical
      \pgfmathsetmacro{\ci@width}{0};
      \pgfmathsetmacro{\imagesize}{\ci@scale * \ci@height};
      \def\ci@imagesizename{height};
      \def\ci@imageanchor{south east};
      \def\ci@ticksanchor{west};
      \def\ci@mtdx{-2.5pt}; % major tick delta x
      \def\ci@mtdy{0};      % major tick delta y
      \def\ci@tdx{-1pt};    % minor tick delta x
      \def\ci@tdy{0};       % minor tick delta y
      \def\ci@facx{0};
      \def\ci@facy{1};
      \def\ci@legendanchor{south};
   }

   % legend image
   \node[anchor=\ci@imageanchor,inner sep=0] (legend) at (\ci@xpos,\ci@ypos) { 
      \includegraphics[\ci@imagesizename=\imagesize cm]{#2} 
   };

   % min tick
   \pgfmathsetmacro{\min}{\ci@min}
   \pgfmathsetmacro{\max}{\ci@max}
   \draw ($(\ci@xpos,\ci@ypos)$)++(\ci@mtdx+\pgflinewidth*\ci@facx,\ci@mtdy+\pgflinewidth*\ci@facy) -- ++(-2*\ci@mtdx,-2*\ci@mtdy) 
      node[anchor=\ci@ticksanchor] {\pgfmathparse{\min}\pgfmathprintnumber{\pgfmathresult}};
   % max tick
   \draw ($(\ci@xpos+\ci@width,\ci@ypos+\ci@height)$)++(\ci@mtdx,\ci@mtdy) -- ++(-2*\ci@mtdx,-2*\ci@mtdy) 
      node[anchor=\ci@ticksanchor] {\pgfmathparse{\max}\pgfmathprintnumber{\pgfmathresult}};

   % major ticks
   \pgfmathsetmacro{\mtics}{\ci@mtics}
   \pgfmathsetmacro{\tics}{\ci@tics}
   \pgfmathsetmacro{\tmin}{( ceil(\ci@min/\ci@tics)*\ci@tics)}
   \pgfmathsetmacro{\tmax}{(floor(\ci@max/\ci@tics)*\ci@tics)}
   \pgfmathparse{\tmin < \min+2*\mtics ? \tmin+\tics : \tmin}
   \pgfmathsetmacro{\tmin}{\pgfmathresult}
   \pgfmathparse{\tmax > \max-2*\mtics ? \tmax-\tics : \tmax}
   \pgfmathsetmacro{\tmax}{\pgfmathresult}
   \pgfmathsetmacro{\tminPtics}{\tmin+\tics}
   \pgfmathsetmacro{\mpt}{ceil((\ci@tics-0.01*\ci@mtics)/\ci@mtics)-1} % miniticks per ticks -1

   \foreach \tick in {\tmin,\tminPtics,...,\tmax} {
      \pgfmathsetmacro{\deltax}{(\tick-\ci@min)/(\ci@max-\ci@min)*\ci@width}
      \pgfmathsetmacro{\deltay}{(\tick-\ci@min)/(\ci@max-\ci@min)*\ci@height}
      \draw ($(\ci@xpos+\deltax,\ci@ypos+\deltay)$)++(\ci@mtdx,\ci@mtdy) -- ++(-2*\ci@mtdx,-2*\ci@mtdy) 
         node[anchor=\ci@ticksanchor] {\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}};

      \pgfmathsetmacro{\upperBound}{int((\max-\tick)/\ci@mtics)}
      \foreach \i in {1,2,...,\mpt} {
         \pgfmathparse{\i <= \upperBound ? 1 : 0}
         \ifthenelse{\equal{\pgfmathresult}{1}}{
            \pgfmathsetmacro{\mdeltax}{(\tick+\i*\mtics-\ci@min)/(\ci@max-\ci@min)*\ci@width}
            \pgfmathsetmacro{\mdeltay}{(\tick+\i*\mtics-\ci@min)/(\ci@max-\ci@min)*\ci@height}
            \draw ($(\ci@xpos+\mdeltax,\ci@ypos+\mdeltay)$)++(\ci@tdx,\ci@tdy) -- ++(-2*\ci@tdx,-2*\ci@tdy);
         }{}
      }

   }
   \pgfmathsetmacro{\upperBound}{ceil((\tmin-\min-0.01*\mtics)/\ci@mtics)-1}
   \foreach \i in {1,2,...,\mpt} {
      \pgfmathparse{\i <= \upperBound ? 1 : 0}
      \ifthenelse{\equal{\pgfmathresult}{1}}{
         \pgfmathsetmacro{\mdeltax}{(\tmin-\i*\mtics-\ci@min)/(\ci@max-\ci@min)*\ci@width}
         \pgfmathsetmacro{\mdeltay}{(\tmin-\i*\mtics-\ci@min)/(\ci@max-\ci@min)*\ci@height}
         \draw ($(\ci@xpos+\mdeltax,\ci@ypos+\mdeltay)$)++(\ci@tdx,\ci@tdy) -- ++(-2*\ci@tdx,-2*\ci@tdy);
      }{}
   }

   \@ifundefined{ci@label}{}{
      \draw ($(\ci@xpos,\ci@ypos+\ci@height)$) node[anchor=\ci@legendanchor] {\ci@label};
   }

   \endgroup
}
\makeatother

